Spatiotemporal Local Propagation

This paper proposes an in-depth re-thinking of neural computation that parallels apparently unrelated laws of physics, that are formulated in the variational framework of the least action principle. The theory holds for neural networks that are also based on any digraph, and the resulting computational scheme exhibits the intriguing property of being truly biologically plausible. The scheme, which is referred to as SpatioTemporal Local Propagation (STLP), is local in both space and time. Space locality comes from the expression of the network connections by an appropriate Lagrangian term, so as the corresponding computational scheme does not need the backpropagation (BP) of the error, while temporal locality is the outcome of the variational formulation of the problem. Overall, in addition to conquering the often invoked biological plausibility missed by BP, the locality in both space and time that arises from the proposed theory can neither be exhibited by Backpropagation Through Time (BPTT) nor by Real-Time Recurrent Learning (RTRL).

==> mechanics.tex <==

\begin{figure}[t]
\[{\|1|\atop\hbox{(a)}}\qquad {\|2|\atop\hbox{(b)}}\]
\vskip -1pc
\caption{Two typical example of holonomic constraints in classical
mechanics: An inclined plane (a) and the
pendulum constraint (b).}
\label{fig-1}
\end{figure}

It turns out the the theory presented in Section~\ref{dirichlet-sec} is
general enough to encompass Classical Mechanics. Indeed if we let $n=1$ and
we regard $x$ as a temporal parameter, when $\varpi(t)=m$ (the mass of
the particle)
with $m>0$ and $F(t,u(t),\dot u(t))=-V(u(t))$ the functional $\S(u)$
is the action of a particle that moves in the potential $V$.

{\bf Example 1} ({\it Inclined Plane}).
Let us consider a simple example in classical mechanics
of a mass sliding on a frictionless inclined plane. The motion takes place on
a two dimensional plane. This correspond to the case, $N=2$.
Let $u^1$ and $u^2$ be the coordinates of the mass on the plane,
then the action is
\begin{equation}
\S(u)=\int_{t_0}^{t_1}
\Bigl({m\over 2}\vert\dot u\vert^2-mgu\cdot \hat e_2\Bigr)\, dt,\end{equation}
where $\hat e_2=({0\atop 1})$ and g is the value of the gravitational
acceleration.
The constraint here is $G(u)=u\cdot v$ (see Fig.~\ref{fig-1}--(a)), where
$v=({-t\atop 1})$, $t>0$. Therefore we have $G_u(u)=v$, $G_{u^i u^k}\equiv 0$
for all $i=1,2$, $L_F(u)=-mg\hat e_2$. This means that $\lambda=-mg/(1+t^2)$; then
the equations of motion for the mass becomes
\begin{equation}
-\ddot u(t)+{g\over 1+t^2}v-g\hat e_2=0. 
\end{equation}
In order to understand this result intuitively let us consider the rotation
matrix $R(\vartheta)={\cos\vartheta\,-\sin\vartheta\choose\sin\vartheta\,
\cos\vartheta}$ and
consider the change of coordinates $u\mapsto R(-\theta) u=:U$ with
$\theta =\arctan t$ (the slope of the inclined plane), then the Euler
equation in this new reference frame are
\begin{equation}-\ddot U(t)-g\begin{pmatrix}\sin\theta\\
0\end{pmatrix}=0,\end{equation}
which indeed is the well known equation of motion of a mass on an inclined plane
written in the reference frame where $U^1$ is parallel to the plane.

\medskip\noindent
{\bf Example 2} ({\it Pendulum}).
Consider the motion of a particle on a circumference
under the action of gravity (pendulum). The setting is the same as the one
in Example~1; this time however the constraint is quadratic: $G(u)=
{1\over 2}\vert u\vert^2-\ell u\cdot \hat e_2$ (Fig.~\ref{fig-1}--(b)).
 Therefore $G_u(u)=u-\ell\hat e_2$ and
$(G_{u^i u^j})={1\,0\choose0\,1}$, then
\begin{equation}\lambda=m {\vert\dot u\vert^2+g(l-u\cdot \hat e_2)\over
\vert u\vert^2-2lu\cdot\hat e_2+\ell^2}.\end{equation}
Thus the non-linear Euler equation reads
\begin{equation}-\ddot u(t)- {\vert \dot u(t)\vert^2+g(\ell-u(t)\cdot \hat e_2)\over
\vert u(t)\vert^2-2\ell u(t)\cdot\hat e_2+\ell^2}(u(t)-\ell\hat e_2)-g\hat e_2=0,
\end{equation}
this is indeed the awkward form that arises
in Cartesian coordinates of the non-linear equation 
of the pendulum, that in polar coordinates assumes the well known form $\ell \ddot \theta+g\sin\theta=0$.

% Local Variables:  
% mode: latex
% TeX-master: "ccal.tex"
% End:
